Memory Tax: Dissecting the Net Value of Agent Memory

Memory is increasingly used in long-horizon agents, yet the net value of building memory over direct retrieval from raw history remains largely unclear. Through a large-scale evaluation across multiple benchmarks and model backbones, we find many dedicated memory systems underperform naive RAG in many cases, indicating a negative net value. Taking RAG as a reference, we dissect the net value of memory into the gains and losses over direct retrieval, termed memory benefit and memory tax. These gains and losses arise because memory process changes how the raw information is organized and accessed. We view such changes as the double-edged deviations from the raw history. They are originally designed and introduced to benefit the task, for example by reorganizing facts or distilling preferences, but some may also remove or obscure evidence, giving rise to memory tax. Since memory benefit reflects the expected gains of its design, we then focus more on the overlooked memory tax, study how it arises from the system and evaluation side, and generalize the concept to more application scenarios of memory. We hope the notion of memory tax can provide a new lens and shift more attention from standalone performance to the net value of memory, informing more reliable memory designs and evaluations. We will open-source the code and results to the community. Project Page: https://hexuan21.github.io/MemoryTax/

==> Tables/faithfulness.tex <==
% Faithfulness (Section 4.2): answer each question from its oracle raw chunks (RAG-1rd row) vs. from each system's
% oracle memory units built from those chunks; the accuracy gap measures information lost in construction.
% Raw Item = the Oracle row of update_4B.txt / update_27B.txt (Q3.5-4B 73.40 / 58.67, Q3.6-27B 84.60 / 72.91; LME after the 10-05 v3-pref re-run, was 72.00 / 83.40); MINT dropped (10-04 user).
% Gold-memory-unit rows (10-05 user run): MemOS 65.40 / 79.80 / 52.68 / 70.45, PlugMem 58.80 / 65.80 / 46.90 / 46.25,
% MAGMA 56.80 / 67.80 / 53.85 / 71.63 (LME Q4B / Q27B, PM Q4B / Q27B); SimpleMem / MemoryOS / LightMem pending.
% 10-05: gold-memory-unit rows from analysis/1_faithfulness/oracle_mem_ablation.txt (single source from now on;
% MemoryOS oracle = raw, it keeps the raw pages). SimpleMem / LightMem not run.
\begin{table}[ht]   % 10-05: in C.2, stays next to its text when possible
\centering
\caption{QA accuracy (\%) when answering from either the original gold raw turns or the corresponding gold memory units constructed by each memory system.}
\vspace{-0.7em}
\label{tab:faithfulness}
\small
\setlength{\tabcolsep}{6pt}   % 10-04: capped at the column width (adjustbox)
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c@{\hspace{2pt}}l cc cc}
\toprule
% 10-04 user: MINT dropped; each benchmark split into the two Qwen backbones
\multicolumn{2}{l}{\multirow{2}{*}{\textbf{Oracle Source}}} & \multicolumn{2}{c}{\textbf{LongMemEval-s}} & \multicolumn{2}{c}{\textbf{PersonaMem-v2}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{l}{} & \textbf{\texttt{Q4B}} & \textbf{\texttt{Q27B}} & \textbf{\texttt{Q4B}} & \textbf{\texttt{Q27B}} \\   % 10-04 user: short bold names as in Table 1
\midrule
\multicolumn{2}{l}{\textit{Raw Item}} & \textit{73.4} & \textit{84.6} & \textit{58.7} & \textit{72.9} \\   % 10-05 user: italic row
\midrule
% 10-03 user: class icon (as in Table 1) spanning each group's rows, no class name
\multirow{2}{*}{\clsFlat} & \textsc{MemOS} & 65.4 & 79.8 & 52.7 & 70.5 \\
                          & \textsc{SimpleMem}  & & & & \\
\arrayrulecolor{black!30}\midrule\arrayrulecolor{black}   % 10-03 user: grey separator between memory types
% & \textsc{OpenViking} & & & & \\
\multirow{2}{*}{\clsHier} & \textsc{MemoryOS} & 73.4 & 84.6 & 58.7 & 72.9 \\
& \textsc{LightMem}   & & & & \\
\arrayrulecolor{black!30}\midrule\arrayrulecolor{black}   % 10-03 user: grey separator between memory types
\multirow{2}{*}{\clsGraph} & \textsc{PlugMem} & 73.2 & 79.6 & 53.6 & 63.7 \\
                           & \textsc{MAGMA} & 56.8 & 67.8 & 53.9 & 71.6 \\
\arrayrulecolor{black!30}\midrule\arrayrulecolor{black}   % 10-05 user: + Trained Policy (as Table 1)
\multirow{2}{*}{\clsTrain} & \textsc{Mem-T} & 60.6 & 67.6 & 40.4 & 50.4 \\
                           & \textsc{Memory-R2} & 67.0 & 73.6 & 51.5 & 68.2 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-0.5em}
\end{table}


==> Tables/generalization.tex <==
\begin{table}[H]
\centering
\caption{\todo{} Experiential memory on agentic benchmarks with backbone \texttt{Qwen3.5-4B}. Cells are shaded in proportion to how far they \colorbox{DegOrange!30}{fall below} or \colorbox{ImpGreen!30}{rise above} Naive RAG. See details in Appendix~\ref{apdx:generalization}.}
\label{tab:generalization}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Embodied} & \textbf{Web} & \textbf{Coding} & \multicolumn{2}{c}{\textbf{Tools}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6}
 & \textbf{ALFWorld} & \textbf{Mind2Web} & \textbf{BigCodeBench} & \textbf{AppWorld} & \textbf{$\tau^2$-Bench} \\
\midrule
No Memory & 52.2 & 48.5 & 16.9 & 12.5 & 61.0 \\
Naive RAG & 73.1 & 45.3 & \textbf{21.6} & \textbf{22.6} & 69.0 \\
\midrule
\textsc{ExpeL} &  &  &  &  &  \\
\textsc{G-Memory} & \cellcolor{ImpGreen!10}73.9 & \cellcolor{ImpGreen!11}47.0 & \cellcolor{DegOrange!11}20.3 & \textbf{22.6} & \cellcolor{ImpGreen!26}\textbf{78.0} \\
\textsc{Mem}$^p$ & \cellcolor{ImpGreen!14}\textbf{76.1} & \cellcolor{ImpGreen!13}47.9 & \cellcolor{DegOrange!11}20.3 & \cellcolor{DegOrange!25}14.3 & \cellcolor{DegOrange!22}62.0 \\
\textsc{ReaBank}$^\dagger$ & \cellcolor{DegOrange!29}62.7 & \cellcolor{ImpGreen!17}\textbf{49.9} & \cellcolor{DegOrange!21}14.9 & \cellcolor{DegOrange!25}14.3 & \cellcolor{DegOrange!44}51.0 \\
\bottomrule
\end{tabular}%
}
\par\vspace{2pt}\raggedright\footnotesize $^\dagger$Short for \textsc{ReasoningBank}.
\end{table}


==> Tables/regimes.tex <==
% Retrieval-only controls across the exploratory benchmarks (rethink_user_mem/explore.txt).
% A single-column table in the ACL two-column layout (was a wraptable in the ICLR version).
% Benchmarks are ordered by the RAG (1rd) score and stacked in blocks.
% Regenerate with scratchpad/gen_regimes.py.
\begin{table}[t]
\centering
\caption{Two retrieval-only controls across benchmarks, ordered by the score of RAG (1rd). Backbone \texttt{Qwen3.6-27B}; all other settings follow Section~\ref{sec:exp_setup}. Scores are judge accuracy (\%); SubtleMemory and EverMemBench are multiple choice and report exact match. Retrieval budgets and coverage are in Appendix~\ref{apdx:regimes}.}
\label{tab:regimes}
\small
\setlength{\tabcolsep}{3pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l c c c}
\toprule
\textbf{Method} & \textbf{SubtleMemory} & \textbf{EverMemBench} & \textbf{ConvoMem} \\
\midrule
IDF-retrieval (1rd) & 83.0 & 68.2 & 52.6 \\
RAG (1rd) & 86.2 & 82.7 & 81.9 \\
\midrule
\textbf{Method} & \textbf{HaluMem} & \textbf{LoCoMo} & \textbf{GroupMemBench} \\
\midrule
IDF-retrieval (1rd) & 51.2 & 56.2 & 29.4 \\
RAG (1rd) & 77.1 & 69.2 & 53.7 \\
\midrule
\textbf{Method} & \textbf{KnowMe-Bench} & \textbf{BEAM} & \textbf{RealMem} \\
\midrule
IDF-retrieval (1rd) & 17.3 & 25.9 & 15.6 \\
RAG (1rd) & 43.7 & 43.6 & 21.1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> Tables/regimes_generalization.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/4_bench_saturate.pdf}
\par\vspace{-0.7em}
\caption{Simple retrieval baselines across different memory benchmarks with \texttt{Qwen3.6-27B}. \faImage[regular]~marks multimodal benchmarks. Full details are in Appendix~\ref{apdx:regimes}.}
\label{fig:regimes}
\vspace{-1.0em}
\end{figure}


==> Tables/venn_all.tex <==
% Appendix C.1: per-query correctness overlap with RAG (1rd), full width (10-02 user): one row per main benchmark,
% Qwen3.6-27B left / GPT-5.6 Luna right. Images: analysis/venn/figs/{27b,luna}.
\begin{figure*}[b]   % 10-02 user: bottom of the page (stfloats)
\centering
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_longmemeval_s_27b.png}\hfill
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_longmemeval_s_luna.png}\\[0.4em]
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_persona_mem_v2_128k_27b.png}\hfill
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_persona_mem_v2_128k_luna.png}\\[0.4em]
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_mint_eval_s_27b.png}\hfill
\includegraphics[width=0.495\textwidth]{Figures/apdx_venn_mint_eval_s_luna.png}
\caption{Per-query correctness overlap between each memory system and RAG (1rd) on LongMemEval-s, PersonaMem-v2 and MINT-Eval (rows), with \texttt{Qwen3.6-27B} (left) and \texttt{GPT-5.6 Luna} (right; LongMemEval-s: 100-question subset).}
\label{fig:venn_all}
\end{figure*}

